State Space Model of Realized Volatility under the Existence of Dependent Market Microstructure Noise

Volatility means the degree of variation of a stock price which is important in finance. Realized Volatility (RV) is an estimator of the volatility calculated using high-frequency observed prices. RV has lately attracted considerable attention of econometrics and mathematical finance. However, it is known that high-frequency data includes observation errors called market microstructure noise (MN). Nagakura and Watanabe[2015] proposed a state space model that resolves RV into true volatility and influence of MN. In this paper, we assume a dependent MN that autocorrelates and correlates with return as reported by Hansen and Lunde[2006] and extends the results of Nagakura and Watanabe[2015] and compare models by simulation and actual data.

==> Proofs.tex <==
\begin{prf}[定理\ref{ret_property}]
以降,上付き添え字の$(m)$は省略する.

伊藤積分の期待値は0なので
\begin{align*}
\E[p(t)]=\E[r_t]=0.
\end{align*}

以降, 計算のため, $e_t$を次のように表す.
\begin{align}
\intertext{$e_t$の定義より,}
e_t&=\eps_t-\eps_{t-\frac{1}{m}}\nonumber\\
\intertext{仮定\ref{assum_ma_corp}, $\eps_t$の定義より,}
&=e^{(1)}_t+e^{(2)}_t+\delta_t'.\nonumber
\end{align}
ただし, 
\begin{align}
e^{(1)}_t&=f(m)\left[\int^t_{t-\frac{1}{m}}dW(s)-\int^{t-\frac{1}{m}}_{t-\frac{2}{m}}dW(s)\right],\\
e^{(2)}_t&=\sum^{q+1}_{i=0}(\Psi_i-\Psi_{i-1})\zeta_{t-i}, \Psi_{-1}=\Psi_{q+1}=0,\\
\delta_t'&=\delta_t-\delta_{t-\frac{1}{m}}.
\end{align}
これらの自己共分散は次のようになる.
\begin{align}
\label{vare1}
\V[e^{(1)}_t]&=\cfrac{2(f(m))^2}{m},\\
\label{vare2}
 \V[e^{(2)}_t]&=2\sum^{q+1}_{i=0}(\Psi_i-\Psi_{i-1})^2\sigma_\zeta^2=2(\Omega_0-\Omega_1),\\
 \label{vare3}
  \V[\delta_t']&=2\sigma_\delta^2,\\
  \label{cove1}
  \E[e^{(1)}_te^{(1)}_{t\pm\frac{n}{m}}]&=
  \begin{cases}
  -\cfrac{(f(m))^2}{m}&(n=1),\\
  0&(n\geq 2),
  \end{cases}\\
  \label{cove2}
  \E[e^{(2)}_te^{(2)}_{t\pm\frac{n}{m}}]&=\sum^{q+1-n}_{i=0}(\Psi_i-\Psi_{i-1})(\Psi_{i+n}-\Psi_{i+n-1})\sigma_\zeta^2=2\Omega_n-\Omega_{n-1}-\Omega_{n+1},\\
  \label{cove3}
  \E[\delta_t'\delta_{t\pm\frac{n}{m}}']&=
   \begin{cases}
  -\sigma_\delta^2&(n=1),\\
  0&(n\geq 2).
  \end{cases}
\end{align}



式(\ref{covreps})から,
\begin{align*}
\cov[r_s, e_t]=
\begin{cases}
\cfrac{f(m)\E[\sigma(t)]}{m}&(t=s),\\
0&(t\neq s).
\end{cases}
\end{align*}

また, 
\begin{align*}
\E[p^*(t)]&=\E[r_t^*]=\E[e_t]=0,\\
\intertext{式(\ref{vare1}), (\ref{vare2}), (\ref{vare3})から,}
\V[e_t]&=\E\left[e_t^2\right]\\
&=\E[e^{(1)2}_t]+\E[e^{(2)2}_t]+\E[e^{(3)2}_t]\\
&=2\left(\cfrac{(f(m))^2}{m}+\Omega_0-\Omega_1+\sigma_\delta^2\right),\\
\V[r_t^*]&=\V[r_t+e_t]\nonumber \\
&=\V[r_t]+\V[e_t]+2\cov[r_t, e_t]\nonumber \\
&= \V \left[p(t)-p\left(t-1/m\right)\right]+\V[e_t]+2\cov[r_t, e_t]\\
&=\V \left[\int^t_{t-1/m}\sigma(s)dW(s)\right]+\V[e_t]+2\cov[r_t, e_t]\\
&=\E\left[\left(\int^t_{t-1/m}\sigma(s)dW(s)\right)^2\right]+\V[e_t]+2\cov[r_t, e_t]\\
\intertext{伊藤の等長性より,}
&=\E\left[\int^t_{t-1/m}\sigma^2(s)ds\right]+\V[e_t]+2\cov[r_t, e_t]\\
\intertext{Fubiniの定理により,}
&=\int^t_{t-1/m}\E[\sigma^2(s)]ds+\V[e_t]+2\cov[r_t, e_t]\\
&=\cfrac{\sigma^2}{m}+2\left(\cfrac{(f(m))^2}{m}+\Omega_0-\Omega_1+\sigma_\delta^2\right)+\cfrac{f(m)\E[\sigma(t)]}{m}.
\end{align*}

$r_s\indepe e^{(2)}_t \delta_t, \forall s,t$だから, 式(\ref{covreps})から,
\begin{align*}
\E\left[r_te_{t-\frac{n}{m}}\right]&=\E\left[r_te^{(1)}_{t-\frac{n}{m}}\right]=0\qquad(n\geq 1)、\\
\E\left[r_te_{t+\frac{n}{m}}\right]&=\E\left[r_te^{(1)}_{t+\frac{n}{m}}\right]=
\begin{cases}
\cfrac{f(m)\E[\sigma(t)]}{m}&(n=1),\\
0&(n\geq 2).
\end{cases}
\end{align*}

式(\ref{cove1}), (\ref{cove2}), (\ref{cove3})から,
\begin{align}
\cov[e_t, e_{t\pm\frac{n}{m}}]=
\begin{cases}
  -\cfrac{(f(m))^2}{m}+2\Omega_1-\Omega_0-\Omega_2-\sigma_\delta^2&(n=1),\\
  2\Omega_n-\Omega_{n-1}-\Omega_{n+1}&(n\geq 2).
  \end{cases}
\end{align}
これらから, 観測リターン$r^*_t$の自己共分散が次で得られる.
\begin{align}
\label{acvr*}
\cov\left[r^*_t, r^*_{t-n/m}\right]&=\E\left[r^*_tr^*_{t-n/m}\right]-\E\left[r^*_t\right]\E\left[r^*_{t-n/m}\right]\nonumber\\
&=\E\left[r_tr_{t-n/m}+r_te_{t-n/m}+r_{t-n/m}e_{t}+e_{t}e_{t-n/m}\right] \nonumber\\
&=\E\left[r_{t}e_{t+n/m}\right]+\E\left[e_{t}e_{t-n/m}\right] \nonumber\\
&=
\begin{cases}
  \cfrac{f(m)\E[\sigma(t)]}{m}-\cfrac{(f(m))^2}{m}+2\Omega_1-\Omega_0-\Omega_2-\sigma_\delta^2&(n=1),\\
  2\Omega_n-\Omega_{n-1}-\Omega_{n+1}&(n\geq 2).
  \end{cases}
\end{align}
\qed
\end{prf}

%%%%%%%%
\begin{framed}
\begin{lem}
\label{mainlem}
\begin{enumerate}
\item 
\begin{align*}
\epsilon_t=\sum^\infty_{i=0}\varrho_i w_{t-i}, w_t\sim {\rm WN}(\sigma_w^2),  \sum^\infty_{i=0}|\varrho_i|<\infty.
\end{align*}
\item 任意の$t$に対し,
\begin{align*}
&\E\left[w_t^4\right]=:\omega_w^2<\infty, \cov\left[w_s^2, w_t^2\right]=\cov\left[w_s, w_t^3\right]=0, (s\neq t),\\
&\E\left[w_sw_tw_u^2\right]=0, (s\neq t\neq u), \E\left[w_sw_tw_uw_v\right]=0, (s\neq t\neq u\neq v).
\end{align*}
\end{enumerate}
1,2の下, 次が成り立つ.
$a\geq b\geq c\geq d\in \mathbb{Z}$とする.
\begin{align*}
\E\left[\epsilon_{t+a}\epsilon_{t+b}\epsilon_{t+c}\epsilon_{t+d}\right]=\left(\omega_w^2-3\sigma_w^4\right)\sum^\infty_{i=0}\varrho_{i+a-d}\varrho_{i+b-d}\varrho_{i+c-d}\varrho_{i}+\Omega_{c-d}\Omega_{a-b}+\Omega_{b-d}\Omega_{a-c}+\Omega_{a-d}\Omega_{b-c}.
\end{align*}
ただし,  $\Omega_k:=\cov[\epsilon_t, \epsilon_{t\pm n}]=\sigma_w^2\sum^\infty_{i=0}\varrho_{i+k}\varrho_i.$
\end{lem}
\end{framed}
\begin{prf}[補題\ref{mainlem}]
\begin{align*}
\E\left[\epsilon_{t+a}\epsilon_{t+b}\epsilon_{t+c}\epsilon_{t+d}\right]&=\E\left[\left(\sum^\infty_{i=0}\varrho_iw_{t+a-i}\right)\left(\sum^\infty_{j=0}\varrho_jw_{t+b-j}\right)\left(\sum^\infty_{k=0}\varrho_kw_{t+c-k}\right)\left(\sum^\infty_{l=0}\varrho_lw_{t+d-l}\right)\right]\\
&=\E\left[\left(\sum^\infty_{i=-a}\varrho_{i+a}w_{t-i}\right)\left(\sum^\infty_{j=-b}\varrho_{j+b}w_{t-j}\right)\left(\sum^\infty_{k=-c}\varrho_{k+c}w_{t-k}\right)\left(\sum^\infty_{l=-d}\varrho_{l+d}w_{t-l}\right)\right]
\end{align*}
仮定から$({\rm i})w_t^4, (\ii)w_t^2w_s^2$の項のみ考えればよい.
\begin{description}
\item[({\rm i})]$w_t^4$の係数\\
$i=j=k=l$のとき係数は$\varrho_{i+a}\varrho_{i+b}\varrho_{i+c}\varrho_{i+d} \qquad(i\geq-d)$
\item[(\ii)]$w_t^2w_s^2$の係数\\
\begin{itemize}
\item $i=j\neq k=l$のとき係数は$\varrho_{i+a}\varrho_{i+b}\varrho_{k+c}\varrho_{k+d} \qquad(i\geq-b, k\geq-d)$
\item $i=k\neq l=j$のとき係数は$\varrho_{i+a}\varrho_{i+c}\varrho_{j+b}\varrho_{j+d} \qquad(i\geq-c, j\geq-d)$
\item $i=l\neq k=j$のとき係数は$\varrho_{i+a}\varrho_{i+d}\varrho_{j+b}\varrho_{j+c} \qquad(i\geq-d, j\geq-c)$
\end{itemize}
\end{description}
よって,
\begin{align*}
&\E\left[\left(\sum^\infty_{i=-a}\varrho_{i+a}w_{t-i}\right)\left(\sum^\infty_{j=-b}\varrho_{j+b}w_{t-j}\right)\left(\sum^\infty_{k=-c}\varrho_{k+c}w_{t-k}\right)\left(\sum^\infty_{l=-d}\varrho_{l+d}w_{t-l}\right)\right]\\
&=\E\left[\sum^\infty_{i=-d}\varrho_{i+a}\varrho_{i+b}\varrho_{i+c}\varrho_{i+d}w_{t-i}^4\right]+\E\left[\sum^\infty_{k=-d}\varrho_{k+c}\varrho_{k+d}\left(\sum^\infty_{i=-b}\varrho_{i+a}\varrho_{i+b}-\varrho_{k+a}\varrho_{k+b}\right)w_{t-i}^2w_{t-k}^2 \right.\\
&\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad+\sum^\infty_{i=-d}\varrho_{i+b}\varrho_{i+d}\left(\sum^\infty_{j=-c}\varrho_{j+a}\varrho_{j+v}-\varrho_{i+a}\varrho_{i+c}\right)w_{t-j}^2w_{t-i}^2\\
&\left.\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad+\sum^\infty_{i=-d}\varrho_{i+a}\varrho_{i+d}\left(\sum^\infty_{j=-c}\varrho_{j+b}\varrho_{j+c}w_{t-i}^2-\varrho_{i+b}\varrho_{i+c}\right)w_{t-i}^2w_{t-j}^2\right]\\
&=\omega_w^2\sum^\infty_{i=-d}\varrho_{i+a}\varrho_{i+b}\varrho_{i+c}\varrho_{i+d}+\sigma_w^4\left[\sum^\infty_{k=-d}\varrho_{k+c}\varrho_{k+d}\left(\sum^\infty_{i=-b}\varrho_{i+a}\varrho_{i+b}-\varrho_{k+a}\varrho_{k+b}\right) \right.\\
&\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad+\sum^\infty_{i=-d}\varrho_{i+b}\varrho_{i+d}\left(\sum^\infty_{j=-c}\varrho_{j+a}\varrho_{j+c}-\varrho_{i+a}\varrho_{i+c}\right)\\
&\left.\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad+\sum^\infty_{i=-d}\varrho_{i+a}\varrho_{i+d}\left(\sum^\infty_{j=-c}\varrho_{j+b}\varrho_{j+c}-\varrho_{i+b}\varrho_{i+c}\right)\right]\\
&=\left(\omega_w^2-3\sigma_w^4\right)\sum^\infty_{i=-d}\varrho_{i+a}\varrho_{i+b}\varrho_{i+c}\varrho_{i+d}\\
&\qquad+\sigma_w^4\left[\sum^\infty_{k=-d}\varrho_{k+c}\varrho_{k+d}\sum^\infty_{i=-b}\varrho_{i+a}\varrho_{i+b}+\sum^\infty_{i=-d}\varrho_{i+b}\varrho_{i+d}\sum^\infty_{j=-c}\varrho_{j+a}\varrho_{j+c}+\sum^\infty_{i=-d}\varrho_{i+a}\varrho_{i+d}\sum^\infty_{j=-c}\varrho_{j+b}\varrho_{j+c}\right]\\
&=\left(\omega_w^2-3\sigma_w^4\right)\sum^\infty_{i=0}\varrho_{i+a-d}\varrho_{i+b-d}\varrho_{i+c-d}\varrho_{i}+\Omega_{c-d}\Omega_{a-b}+\Omega_{b-d}\Omega_{a-c}+\Omega_{a-d}\Omega_{b-c}.
\end{align*}
\qed
\end{prf}
%%%%%%%%%
%
\newpage
%
\begin{framed}
\begin{lem}
\label{lem2}
$\Delta_i(t)$は$\mathcal{F}(t)$-適合過程とし, $\displaystyle \E\left[\int^t_0\Delta_i^2(s)ds\right]<\infty,\  (i=1,2,3,4)$を仮定する.
$s\leq t-h_2, h_1,h_2>0$とする.
\begin{align*}
&\E\left[\int^s_{s-h_1}\Delta_1(u)dW(u)\int^s_{s-h_1}\Delta_2(u)dW(u)\int^t_{t-h_2}\Delta_3(u)dW(u)\int^t_{t-h_2}\Delta_4(u)dW(u)\right]\\
=&\E\left[\int^s_{s-h_1}\Delta_1(u)\Delta_2(u)du\int^t_{t-h_2}\Delta_3(u)\Delta_4(u)du\right].\\
\intertext{$h>0$とする.}
&\E\left[\int^t_{t-h}\Delta_1(u)dW(u)\int^t_{t-h}\Delta_2(u)dW(u)\int^t_{t-h}\Delta_3(u)dW(u)\int^t_{t-h}\Delta_4(u)dW(u)\right]\\
=&\E\left[\int^t_{t-h}\Delta_1(u)\Delta_2(u)du\int^t_{t-h}\Delta_3(u)\Delta_4(u)du\right.\\
&\qquad+\int^t_{t-h}\Delta_1(u)\Delta_3(u)du\int^t_{t-h}\Delta_2(u)\Delta_4(u)du\\
&\qquad\left.+\int^t_{t-h}\Delta_1(u)\Delta_4(u)du\int^t_{t-h}\Delta_2(u)\Delta_3(u)du\right].
\end{align*}
\end{lem}
\end{framed}
\begin{prf}
積分区間$[s-h_1, s], [t-h_2, t]$を$s-h_1=s_0\leq s_1\leq \cdots \leq s_n=s, t-h_2=t_0\leq t_1\leq \cdots \leq t_n=t$により分割する. $D_{t_i}=W(t_{i+1})-W(t_{i})$とすると,
\begin{align*}
&\E\left[\int^s_{s-h_1}\Delta_1(u)dW(u)\int^s_{s-h_1}\Delta_2(u)dW(u)\int^t_{t-h_2}\Delta_3(u)dW(u)\int^t_{t-h_2}\Delta_4(u)dW(u)\right]\\
\intertext{ここで極限を一つにまとめ, 優収束定理より極限と期待値の順序を交換すると,}
=&\lim_{\max_{i}|s_{i+1}-s_i|\to 0\atop \max_{j}|t_{j+1}-t_j|\to 0}\E\left[\sum^{n-1}_{i=0}\Delta_1(s_i) D_{s_i}\sum^{n-1}_{j=0}\Delta_2(s_j) D_{s_j}\sum^{n-1}_{k=0}\Delta_3(t_k) D_{t_k}\sum^{n-1}_{l=0}\Delta_4(t_l) D_{t_l}\right]\\
\intertext{$[s-h_1, s]\cap[t-h_2, t]=\emptyset$より, $\forall i,j\in[0, n-1], D_{s_i}\indepe D_{t_j}$だから,}
=&\lim_{\max_{i}|s_{i+1}-s_i|\to 0\atop \max_{j}|t_{j+1}-t_j|\to 0}\E\left[\sum^{n-1}_{i=0}\sum^{n-1}_{j=0}\Delta_1(s_i)\Delta_2(s_j) D_{s_i}^2\Delta_3(t_i)\Delta_4(t_j) D_{t_j}^2\right]\\
\intertext{$D_{s_j}, D_{t_j}$は$\mathcal{F}(s_j), \mathcal{F}(t_i)$と独立だから,}
=&\lim_{\max_{i}|s_{i+1}-s_i|\to 0\atop \max_{j}|t_{j+1}-t_j|\to 0}\E\left[\sum^{n-1}_{i=0}\sum^{n-1}_{j=0}\Delta_1(s_i)\Delta_2(s_j)\Delta_3(t_i)\Delta_4(t_j)\right]\E\left[D_{s_i}^2\right]\E\left[D_{t_j}^2\right]\\
=&\E\left[\int^s_{s-h_1}\Delta_1(u)\Delta_2(u)du\int^t_{t-h_2}\Delta_3(u)\Delta_4(u)du\right].
\end{align*}
かくして補題の第1式が示された.次に第2式を示す.
\begin{align*}
&\E\left[\int^t_{t-h}\Delta_1(u)dW(u)\int^t_{t-h}\Delta_2(u)dW(u)\int^t_{t-h}\Delta_3(u)dW(u)\int^t_{t-h}\Delta_4(u)dW(u)\right]\\
=&\lim_{\max_{j}|t_{j+1}-t_j|\to 0}\E\left[\sum^{n-1}_{i=0}\Delta_1(t_i) D_{t_i}\sum^{n-1}_{j=0}\Delta_2(t_j) D_{t_j}\sum^{n-1}_{k=0}\Delta_3(t_k) D_{t_k}\sum^{n-1}_{l=0}\Delta_4(t_l) D_{t_l}\right]\\
=&\lim_{\max_{j}|t_{j+1}-t_j|\to 0}\E\left[\sum^{n-1}_{i=0}\Delta_1(t_i)\Delta_2(t_i)\Delta_3(t_i)\Delta_4(t_i) D_{t_i}^4\right.\\
&\qquad\left.+\sum^{n-1}_{i=0}\sum^{n-1}_{j=0\atop j\neq i}\Delta_1(t_i)\left\{\Delta_2(t_i)\Delta_3(t_j)\Delta_4(t_j)+\Delta_3(t_i)\Delta_2(t_j)\Delta_4(t_j)+\Delta_4(t_i)\Delta_2(t_j)\Delta_3(t_j)\right\}D_{t_i}^2D_{t_j}^2\right].
\end{align*}
ここで, $\displaystyle E_1=\E\left[\sum^{n-1}_{i=0}\Delta_1(t_i)\Delta_2(t_i)\Delta_3(t_i)\Delta_4(t_i) D_{t_i}^4\right], $\\$\displaystyle E_2=\E\left[\sum^{n-1}_{i=0}\sum^{n-1}_{j=0\atop j\neq i}\Delta_1(t_i)\left\{\Delta_2(t_i)\Delta_3(t_j)\Delta_4(t_j)+\Delta_3(t_i)\Delta_2(t_j)\Delta_4(t_j)+\Delta_4(t_i)\Delta_2(t_j)\Delta_3(t_j)\right\}D_{t_i}^2D_{t_j}^2\right]$とおく.
\begin{align*}
E_1&=3\sum^{n-1}_{i=0}\E\left[\Delta_1(t_i)\Delta_2(t_i)\Delta_3(t_i)\Delta_4(t_i)\right] (t_{i+1}-t_i)^2\\
&\leq 3\max_{j}|t_{j+1}-t_j| \sum^{n-1}_{i=0}\E\left[\Delta_1(t_i)\Delta_2(t_i)\Delta_3(t_i)\Delta_4(t_i)\right] (t_{i+1}-t_i)\\
&\to 0\cdot \int^t_{t-h}\E\left[\Delta_1(s)\Delta_2(s)\Delta_3(s)\Delta_4(s)\right]ds\qquad (\max_{j}|t_{j+1}-t_j|\to0)\\
&=0.\\
\intertext{同様に, $\min_{j}|t_{j+1}-t_j|$を前に出せば, $E_1\geq 0.$従って, $E_1=0.$}
E_2&=\sum^{n-1}_{i=0}\sum^{n-1}_{j=0}\E\left[\Delta_1(t_i)\left\{\Delta_2(t_i)\Delta_3(t_j)\Delta_4(t_j)+\Delta_3(t_i)\Delta_2(t_j)\Delta_4(t_j)+\Delta_4(t_i)\Delta_2(t_j)\Delta_3(t_j)\right\}\right.\\
&\qquad\qquad\qquad\left.-3\Delta_1(t_i)\Delta_2(t_i)\Delta_3(t_i)\Delta_4(t_i)\right](t_{i+1}-t_i)^2\\
&=\E\left[\sum^{n-1}_{i=0}\Delta_1(t_i)\Delta_2(t_i)(t_{i+1}-t_i)\sum^{n-1}_{j=0}\Delta_3(t_j)\Delta_4(t_j)(t_{j+1}-t_j)\right.\\
&\qquad\qquad\left.+\sum^{n-1}_{i=0}\Delta_1(t_i)\Delta_3(t_i)(t_{i+1}-t_i)\sum^{n-1}_{j=0}\Delta_2(t_j)\Delta_4(t_j)(t_{j+1}-t_j)\right.\\
&\qquad\qquad\left.+\sum^{n-1}_{i=0}\Delta_1(t_i)\Delta_4(t_i)(t_{i+1}-t_i)\sum^{n-1}_{j=0}\Delta_2(t_j)\Delta_3(t_j)(t_{j+1}-t_j)\right.\\
&\qquad\qquad\left.-3\sum^{n-1}_{i=0}\Delta_1(t_i)\Delta_2(t_i)\Delta_3(t_i)\Delta_4(t_i)(t_{i+1}-t_i)^2\right]\\
\intertext{上と同様に第4項は$0$に収束するので}
&=\E\left[\int^t_{t-h}\Delta_1(u)\Delta_2(u)du\int^t_{t-h}\Delta_3(u)\Delta_4(u)du\right.\\
&\qquad+\int^t_{t-h}\Delta_1(u)\Delta_3(u)du\int^t_{t-h}\Delta_2(u)\Delta_4(u)du\\
&\qquad\left.+\int^t_{t-h}\Delta_1(u)\Delta_4(u)du\int^t_{t-h}\Delta_2(u)\Delta_3(u)du\right].
\end{align*}
\qed
\end{prf}
%%%%%%%%
\begin{prf}[定理\ref{thm1}]
まず$\E[u_t]$を計算する.このために$\cov[r_se_s, r_te_t]$を計算しておく.
%C1
\begin{align*}
\cov[r_te_t, r_te_t]&=\E[r_t^2e_t^2]-\left(\E[r_te_t]\right)^2\nonumber \\
&=\E[r_t^2e^{(1)2}_t]+\E[r_t^2]\E[e^{(2)2}_t+\delta^2_t]-\left(\E[r_te^{(1)}_t]\right)^2\nonumber \\
\intertext{補題\ref{lem2}より, }
&=(f(m))^2\E\left[\cfrac{2}{m}\int^t_{t-\frac{1}{m}}\sigma^2(u)du+2\left(\int^t_{t-\frac{1}{m}}\sigma(u)du\right)^2\right]+\E[r_t^2]\E[e^{(2)2}_t+\delta^2_t]-\left(\E[r_te^{(1)}_t]\right)^2\nonumber \\
&=\cfrac{2\sigma^2}{m}(\Omega_0-\Omega_1+\sigma_\delta^2)+(f(m))^2\left(\cfrac{2\sigma^2}{m^2}+2\E\left[\left(\int^t_{t-\frac{1}{m}}\sigma(s)ds\right)^2\right]-\cfrac{\E[\sigma(t)]}{m}\right).
\end{align*}
次に, $n\geq 1$として, $\cov\left[r_te_t, r_{t\pm\frac{n}{m}}e_{t\pm\frac{n}{m}}\right]$を計算する.
\begin{align*}
\cov\left[r_te_t, r_{t-\frac{n}{m}}e_{t-\frac{n}{m}}\right]&=\E\left[r_tr_{t-\frac{n}{m}}e_te_{t-\frac{n}{m}}\right]-\E[r_te_t]\E\left[r_{t-\frac{n}{m}}e_{t-\frac{n}{m}}\right]\nonumber\\
&=\E\left[r_tr_{t-\frac{n}{m}}e^{(1)}_te^{(1)}_{t-\frac{n}{m}}\right]-\E[r_te^{(1)}_t]\E\left[r_{t-\frac{n}{m}}e^{(1)}_{t-\frac{n}{m}}\right]\nonumber\\
\intertext{補題\ref{lem2}より,}
&=\E\left[\int^t_{t-\frac{1}{m}}\sigma(u)du\int^{t\pm\frac{n}{m}}_{t\pm\frac{n\pm1}{m}}\sigma(u)du\right]-\E[r_te^{(1)}_t]\E\left[r_{t-\frac{n}{m}}e^{(1)}_{t-\frac{n}{m}}\right]\\
&=(f(m))^2\cov\left[\int^t_{t-\frac{1}{m}}\sigma(s)ds, \int^{t-\frac{n}{m}}_{t-\frac{n+1}{m}}\sigma(s)ds\right].
\end{align*}
同様にして, 
\begin{align}
\label{alpha}
C_n^{(1)}:=\cov\left[r_te_t, r_{t\pm\frac{n}{m}}e_{t\pm\frac{n}{m}}\right]=(f(m))^2\cov\left[\int^t_{t-\frac{1}{m}}\sigma(s)ds, \int^{t\pm\frac{n}{m}}_{t\pm\frac{n\pm1}{m}}\sigma(s)ds\right].
\end{align}


以上から $u_t$の平均は次のようになる.
\begin{align}
\E[u_t]&=2\sum^m_{i=1}\E[r_{t-1+i/m}e_{t-1+i/m}]+\sum^m_{i=1}\E\left[e^2_{t-1+i/m}\right]\nonumber\\
&=\cfrac{f(m)}{m}\sum^m_{i=1}\E\left[\sigma\left(t-1+\frac{i-1}{m}\right)\right]+2m\left(\cfrac{(f(m))^2}{m}+\Omega_0-\Omega_1+\sigma_\delta^2\right)\nonumber\\
&=2m(\Omega_0-\Omega_1+\sigma_\delta^2)+2(f(m))^2+2f(m)\E\left[\sigma(t)\right].
\end{align}　

次に$\V\left[u_t\right], \cov\left[u_t, u_{t\pm n}\right]$を求める.このためにまず, $\cov[r_te_t, e_s^2], \cov[e_s^2, e_t^2]$を計算する.
%C2
\begin{align*}
\cov\left[r_te_t, e_t^2\right]&=\E\left[r_te_t^3\right]-\E\left[r_te_t\right]\E\left[e_t^2\right]\\
&=\E\left[r_te_t^{(1)3}\right]-\E\left[r_te_t^{(1)}\right]\E\left[e_t^{(1)2}\right]+3\E\left[r_te_t^{(1)}\right]\left(\E\left[e_t^{(2)2}\right]+\E\left[\delta_t^2\right]\right)\\
\intertext{補題\ref{lem2}より,}
&=(f(m))^3\E\left[\cfrac{3}{m}\int^t_{t-\frac{1}{m}}\sigma(u)du-\cfrac{3}{m}\int^t_{t-\frac{1}{m}}\sigma(u)du\right]-\E\left[r_te_t^{(1)}\right]\E\left[e_t^{(1)2}\right]\\
&\qquad\qquad+3\E\left[r_te_t^{(1)}\right]\left(\E\left[e_t^{(2)2}\right]+\E\left[\delta_t^2\right]\right)\\
&=\cfrac{2f(m)}{m}\E\left[\sigma(t)\right]\left(-\cfrac{(f(m))^2}{m}+2(\Omega_0-\Omega_1+\sigma_\delta^2)\right).
\end{align*}
\begin{align*}
\cov\left[r_{t-\frac{1}{m}}e_{t-\frac{1}{m}}, e_t^2\right]&=\E\left[r_{t-\frac{1}{m}}e_{t-\frac{1}{m}}^{(1)}e_t^{(1)2}\right]-\E\left[r_{t-\frac{1}{m}}e_{t-\frac{1}{m}}^{(1)}\right]\E\left[e_t^{2}\right]\\
\intertext{補題\ref{lem2}より,}
&=(f(m))^3\E\left[\cfrac{1}{m}\int^{t-\frac{1}{m}}_{t-\frac{2}{m}}\sigma(u)du+\cfrac{3}{m}\int^{t-\frac{1}{m}}_{t-\frac{2}{m}}\sigma(u)du\right]-\E\left[r_{t-\frac{1}{m}}e_{t-\frac{1}{m}}^{(1)}\right]\E\left[e_t^{2}\right]\\
&=\cfrac{2f(m)}{m}\E\left[\sigma(t)\right]\left(-\cfrac{(f(m))^2}{m}-(\Omega_0-\Omega_1+\sigma_\delta^2)\right).
\end{align*}
$n\geq 2$として,
\begin{align*}
\cov\left[r_{t-\frac{n}{m}}e_{t-\frac{n}{m}}, e_t^2\right]&=\E\left[r_{t-\frac{n}{m}}e_{t-\frac{n}{m}}^{(1)}e_t^{(1)2}\right]-\E\left[r_{t-\frac{n}{m}}e_{t-\frac{n}{m}}^{(1)}\right]\E\left[e_t^{(1)2}\right]\\
&=\E\left[r_{t-\frac{n}{m}}e_{t-\frac{n}{m}}^{(1)}\right]\E\left[e_t^{(1)2}\right]-\E\left[r_{t-\frac{n}{m}}e_{t-\frac{n}{m}}^{(1)}\right]\E\left[e_t^{(1)2}\right]\\
&=0.
\end{align*}
以上より,
\begin{align}
\label{beta}
C_n^{(2)}:&=\cov\left[r_{t-\frac{n}{m}}e_{t-\frac{n}{m}}, e^2_t\right]\nonumber\\
&=\E\left[r_te_te^2_{t-\frac{n}{m}}\right]-\E\left[r_te_t\right]\E\left[e^2_{t-\frac{n}{m}}\right]\nonumber\\
&=
\begin{cases}
\cfrac{2f(m)}{m}\E\left[\sigma(t)\right]\left(-\cfrac{(f(m))^2}{m}+2(\Omega_0-\Omega_1+\sigma_\delta^2)\right)&(n=0),\\
\cfrac{2f(m)}{m}\E\left[\sigma(t)\right]\left(-\cfrac{(f(m))^2}{m}-(\Omega_0-\Omega_1+\sigma_\delta^2)\right)&(n=1),\\
0&(n\geq 2, -1\geq n).
\end{cases}
\end{align}

次に$\cov[e_t^2, e_{t\pm\frac{n}{m}}^2]$を計算していく. $\cov[e_t^{(2)2}, e_{t\pm\frac{n}{m}}^{(2)2}]$は, 補題\ref{mainlem}で$\varrho_i=\Psi_i, (1\leq i\leq q), \varrho_i=0, (i\geq q+1), w_t=\zeta_t\sim N(0,\sigma_\zeta^2)$の場合を考えば良い.  $\zeta_t$は平均$0$の正規分布に従うので, $\omega_w^2=3\sigma_w^4$となり, 補題\ref{mainlem}の第1項が消えることに注意する.
\begin{align*}
\cov[e_t^{(2)2}, e_t^{(2)2}]&=\E[e^{(2)4}_t]-(\E[e_t^{(2)2}])^2 \\
&=\E[\eps^{(2)4}_t-4\eps^{(2)3}_t\eps^{(2)}_{t-1}+6\eps^{(2)2}_t\eps^{(2)2}_{t-1}-4\eps^{(2)}_t\eps^{(2)3}_{t-1}+\eps^{(2)4}_{t-1}]-4(\Omega_0-\Omega_1)^2 \\
&=\E[\eps^{(2)4}_t]-4\E[\eps^{(2)3}_t\eps^{(2)}_{t-1}]+6\E[\eps^{(2)2}_t\eps^{(2)2}_{t-1}]-4\E[\eps^{(2)}_t\eps^{(2)3}_{t-1}]+\E[\eps^{(2)4}_{t-1}]-4(\Omega_0-\Omega_1)^2.\\
\end{align*}

補題\ref{mainlem}から,
\begin{align*}
\E\left[\eps^{(2)4}_t\right]=3\Omega_0^2, \E\left[\eps^{(2)2}_t\eps^{(2)2}_{t-1}\right]=\Omega_0^2+2\Omega_1^2, \E\left[\eps^{(2)3}_t\eps^{(2)}_{t-1}\right]=3\Omega_0\Omega_1, \E\left[\eps^{(2)}_t\eps^{(2)3}_{t-1}\right]=3\Omega_0\Omega_1.
\end{align*}
よって,
\begin{align*}
\cov[e_t^{(2)2}, e_t^{(2)2}]&=\E[\eps^{(2)4}_t]-4\E[\eps^{(2)3}_t\eps^{(2)}_{t-1}]+6\E[\eps^{(2)2}_t\eps^{(2)2}_{t-1}]-4\E[\eps^{(2)}_t\eps^{(2)3}_{t-1}]+\E[\eps^{(2)4}_{t-1}]-4(\Omega_0-\Omega_1)^2\nonumber \\
&=8(\Omega_0-\Omega_1)^2.
\end{align*}

次に, $e_t^{(2)2}$の自己共分散を導出する.
\begin{align*}
\cov\left[e_t^{(2)2}, e_{t\pm \frac{n}{m}}^{(2)2}\right]&=\E\left[(\eps^{(2)}_t-\eps^{(2)2}_{t-1})(\eps^{(2)}_{t\pm n}-\eps^{(2)2}_{t\pm n-1})\right]-\E\left[e_t^{(2)2}\right]\E\left[e_{t\pm \frac{n}{m}}^{(2)2}\right]\\
&=\E[\eps^{(2)2}_t\eps^{(2)2}_{t\pm n}-2\eps^{(2)2}_t\eps^{(2)}_{t\pm n}\eps^{(2)}_{t\pm n-1}+\eps^{(2)2}_t\eps^{(2)2}_{t\pm n-1}-2\eps^{(2)}_t\eps^{(2)}_{t-1}\eps^{(2)2}_{t\pm n}\\
&\qquad +4\eps^{(2)}_t\eps^{(2)}_{t-1}\eps^{(2)}_{t\pm n}\eps^{(2)}_{t\pm n-1}-2\eps^{(2)}_t\eps^{(2)}_{t-1}\eps^{(2)2}_{t\pm n-1}+\eps^{(2)2}_{t-1}\eps^{(2)2}_{t\pm n} \\
&\qquad -2\eps^{(2)2}_{t-1}\eps^{(2)}_{t\pm n}\eps^{(2)}_{t\pm n-1}+\eps^{(2)2}_{t-1}\eps^{(2)2}_{t\pm n-1}]-4(\Omega_0-\Omega_1)^2.
\end{align*}
補題\ref{mainlem}より,
\begin{align*}
\E\left[\eps^{(2)2}_t\eps^{(2)2}_{t\pm n}\right]&=\Omega_0^2+2\Omega_n^2,\\
 \E\left[\eps^{(2)2}_t\eps^{(2)}_{t+n}\eps^{(2)}_{t+n-1}+\eps^{(2)}_t\eps^{(2)}_{t-1}\eps^{(2)2}_{t+n-1}\right]&=2\left(\Omega_0\Omega_1+2\Omega_{n-1}\Omega_n\right),\\
 \E\left[\eps^{(2)}_t\eps^{(2)}_{t-1}\eps^{(2)2}_{t+n}+\eps^{(2)}_{t+n}\eps^{(2)}_{t+n-1}\eps^{(2)2}_{t-1}\right]&=2\left(\Omega_0\Omega_1+2\Omega_{n+1}\Omega_n\right),\\
 \E\left[\eps^{(2)}_t\eps^{(2)}_{t-1}\eps^{(2)}_{t+n}\eps^{(2)}_{t+n-1}\right]&=\Omega_1^2+\Omega_n^2+\Omega_{n+1}\Omega_{n-1}.
\end{align*}
よって,
\begin{align}
\label{turai}
\gamma_n:=\cov\left[e_t^{(2)2}, e_{t\pm \frac{n}{m}}^{(2)2}\right]&=2(4\Omega_{n}^2+\Omega_{n-1}^2+\Omega_{n+1}^2-4\Omega_{n}\Omega_{n+1}-4\Omega_{n-1}\Omega_{n}+2\Omega_{n-1}\Omega_{n+1}).
\end{align}
\begin{align*}
\cov\left[e_t^2, e_t^2\right]&=\E\left[e_t^4\right]-\left(\E\left[e_t^2\right]\right)^2\\
&=\E\left[e_t^{(1)4}+6e_t^{(1)2}e_t^{(2)2}+6e_t^{(1)2}e_t^{(3)2}+6e_t^{(2)2}e_t^{(3)2}+e_t^{(2)4}+e_t^{(3)4}\right]-\left(\E\left[e_t^2\right]\right)^2\\
&=\E\left[e_t^{(1)4}\right]+6\left(\E\left[e_t^{(1)2}\right]\E\left[e_t^{(2)2}\right]+\E\left[e_t^{(2)2}\right]\E\left[e_t^{(3)2}\right]+\E\left[e_t^{(1)2}\right]\E\left[e_t^{(3)2}\right]\right)\\
&\qquad +\E\left[e_t^{(2)4}\right]+\E\left[e_t^{(3)4}\right]-\E\left[e_t^{2(1)}\right]^2-\E\left[e_t^{2(2)}\right]^2-\E\left[e_t^{2(3)}\right]^2\\
&\qquad -4\left(\E\left[e_t^{(1)2}\right]\E\left[e_t^{(2)2}\right]+\E\left[e_t^{(2)2}\right]\E\left[e_t^{(3)2}\right]+\E\left[e_t^{(1)2}\right]\E\left[e_t^{(3)2}\right]\right)\\
&=2\left(\E\left[e_t^{(1)2}\right]\E\left[e_t^{(2)2}\right]+\E\left[e_t^{(2)2}\right]\E\left[e_t^{(3)2}\right]+\E\left[e_t^{(1)2}\right]\E\left[e_t^{(3)2}\right]\right)+\cov\left[e_t^{2(2)}, e_t^{2(2)}\right]\\
&\qquad +2(\omega_\delta^2+\sigma_\delta^4)+\cfrac{8(f(m))^4}{m^2}\\
&=2\left(\cfrac{4(f(m))^2}{m}(\Omega_0-\Omega_1+\sigma_\delta^2)+4\sigma_\delta^2(\Omega_0-\Omega_1)\right)+8(\Omega_0-\Omega_1)^2+2(\omega_\delta^2+\sigma_\delta^4)+\cfrac{8(f(m))^4}{m^2}\\
&=8\left(\sigma_\delta^2(\Omega_0-\Omega_1)+(\Omega_0-\Omega_1)^2+\cfrac{(f(m))^4}{m^2}+\cfrac{(f(m))^2}{m}(\Omega_0-\Omega_1+\sigma_\delta^2)+
\right)+2(\omega_\delta^2+\sigma_\delta^4).
\end{align*}
\begin{align}
\label{gamma}
C^{(3)}_n:&=\cov\left[e_t^2, e_{t\pm \frac{n}{m}}^2\right]\nonumber\\
&=\E\left[e_t^2e_{t\pm \frac{n}{m}}^2\right]-\V\left[e_t^2\right]\nonumber\\
&=\E\left[\left(e_t^{(1)2}+e_t^{(2)2}+e_t^{(3)2}\right)^2\left(e_{t\pm \frac{n}{m}}^{(1)}+e_{t\pm \frac{n}{m}}^{(2)}+e_{t\pm \frac{n}{m}}^{(3)}\right)^2\right]-\V\left[e_t^2\right]\nonumber\\
&=
\begin{cases}
\cov\left[e_t^{(1)2}, e_{t\pm \frac{1}{m}}^{(1)2}\right]+\cov\left[e_t^{(2)2}, e_{t\pm \frac{1}{m}}^{(2)2}\right]+\cov\left[e_t^{(3)2}, e_{t\pm \frac{1}{m}}^{(3)2}\right]&(n=1),\\
\cov\left[e_t^{(2)2}, e_{t\pm \frac{n}{m}}^{(2)2}\right]&(n\geq 2).
\end{cases}\nonumber\\
\thus C^{(3)}_n&=
\begin{cases}
\gamma_1+\omega_\delta^2-\sigma_\delta^4+\cfrac{4(f(m))^2}{m}&(n=1),\\
\gamma_n&(n\geq 2).
\end{cases}
\end{align}

これらから$\V\left[u_t\right], \cov\left[u_t, u_{t\pm n}\right]$が計算できる.
\begin{align}
\V\left[u_t\right]&=\V\left[2\sum^m_{i=1}r_{t-1+\frac{i}{m}}e_{t-1+\frac{i}{m}}+\sum^m_{i=1}e^2_{t-1+\frac{i}{m}}\right]\nonumber \\
&=4\V\left[\sum^m_{i=1}r_{t-1+\frac{i}{m}}e_{t-1+\frac{i}{m}}\right]+\V\left[\sum^m_{i=1}e^2_{t-1+\frac{i}{m}}\right]\nonumber\\
&\qquad+\cov\left[2\sum^m_{i=1}r_{t-1+\frac{i}{m}}e_{t-1+\frac{i}{m}}, \sum^m_{i=1}e^2_{t-1+\frac{i}{m}}\right]\nonumber \\
&=4\sum^m_{i=1}\sum^m_{j=1}\cov\left[r_{t-1+\frac{i}{m}}e_{t-1+\frac{i}{m}}, r_{t-1+\frac{j}{m}}e_{t-1+\frac{j}{m}}\right]\nonumber\\
&\qquad+\sum^m_{i=1}\sum^m_{j=1}\cov\left[e_{t-1+\frac{i}{m}}^2, e^2_{t-1+\frac{j}{m}}\right]+4\sum^m_{i=1}\sum^m_{j=1}\cov\left[r_{t-1+\frac{i}{m}}e_{t-1+\frac{i}{m}}, e^2_{t-1+\frac{j}{m}}\right]\nonumber\\
&=4mC_0^{(1)}+8\sum^{m-1}_{k=1}(m-k)C^{(1)}_k+4mC_0^{(2)}+4\sum^{m-1}_{k=1}(m-k)C_k^{(2)}+mC^{(3)}_0+2\sum^{m-1}_{k=1}(m-k)C^{(3)}_k.\\
\cov\left[u_t, u_{t\pm n}\right]&=\cov\left[2\sum^m_{i=1}r_{t-n+\frac{i}{m}}e_{t-n+\frac{i}{m}}+\sum^m_{i=1}e^2_{t-n+\frac{i}{m}}, 2\sum^m_{i=1}r_{t+\frac{i}{m}}e_{t+\frac{i}{m}}+\sum^m_{i=1}e^2_{t+\frac{i}{m}}\right]\nonumber \\
&=4\cov\left[\sum^m_{i=1}r_{t-n+\frac{i}{m}}e_{t-n+\frac{i}{m}}, \sum^m_{i=1}r_{t+\frac{i}{m}}e_{t+\frac{i}{m}}\right]
+2\cov\left[\sum^m_{i=1}r_{t+\frac{i}{m}}e_{t+\frac{i}{m}}, \sum^m_{i=1}e^2_{t-n+\frac{i}{m}}\right]
\nonumber\\
&\qquad+2\cov\left[\sum^m_{i=1}r_{t-n+\frac{i}{m}}e_{t-n+\frac{i}{m}}, \sum^m_{i=1}e^2_{t+\frac{i}{m}}\right]
+\cov\left[\sum^m_{i=1}e^2_{t-n+\frac{i}{m}}, \sum^m_{i=1}e^2_{t+\frac{i}{m}}\right]\nonumber\\
&=+4mC^{(1)}_{mn}+4\sum^{m-1}_{k=1}(m-k)(C^{(1)}_{mn+k}+C^{(1)}_{mn-k})+2mC^{(2)}_{mn}\nonumber\\
&\qquad +2\sum^{m-1}_{k=1}(m-k)(C^{(2)}_{mn+k}+C^{(2)}_{mn-k})+mC^{(3)}_{mn}+\sum^{m-1}_{k=1}(m-k)(C^{(3)}_{mn+k}+C^{(3)}_{mn-k}).
\end{align}

\qed
\end{prf}
%%%%%%%%%
\begin{prf}[定理\ref{thm2}]
まず$\cov[IV_t, u_s]$を目標に, 次を計算していく.
$\forall s,t, \Delta>0, \Delta'>0$に対し,
\begin{align*}
&\cov\left[\int^{t}_{t-\Delta}\sigma^2(u)du, e_s\int^{s}_{s-\Delta'}\sigma(u)dW(u)\right]\\
&=\E\left[\int^{t}_{t-\Delta}\sigma^2(u)due_s\int^{s}_{s-\Delta'}\sigma(u)dW(u)\right]-\E\left[\int^{t}_{t-\Delta}\sigma^2(u)du\right]\E\left[e_s\int^{s}_{s-\Delta'}\sigma(u)dW(u)\right]\\
&=f(m)\left(\E\left[\int^{t}_{t-\Delta}\sigma^2(u)du\int^s_{s-\Delta'}dW(u)\int^{s}_{s-\Delta'}\sigma(u)dW(u)\right]\right.\\
&\qquad\qquad\qquad\left.-\E\left[\int^{t}_{t-\Delta}\sigma^2(u)du\right]\E\left[\int^s_{s-\Delta'}dW(u)\int^{s}_{s-\Delta'}\sigma(u)dW(u)\right]\right)\\
&=f(m)\left(\E\left[\int^{t}_{t-\Delta}\sigma^2(u)du\int^s_{s-\Delta'}\sigma(u)du\right]-\E\left[\int^{t}_{t-\Delta}\sigma^2(u)du\right]\E\left[\int^{s}_{s-\Delta'}\sigma(u)du\right]\right)\\
&=f(m)\cov\left[\int^{t}_{t-\Delta}\sigma^2(u)du, \int^s_{s-\Delta'}\sigma(u)du\right].
\end{align*}
\begin{align*}
\cov\left[\int^{t}_{t-\Delta}\sigma^2(u)du, e_s^2\right]=0. \qquad\because \sigma^2(t)\indepe e_s.
\end{align*}
以上より,
\begin{align}
\label{ivu}
&\cov[IV_t, u_{t\pm n}]\nonumber\\
&=\cov\left[\sum^m_{i=1}\int^{t-1+\frac{i}{m}}_{t-1+\frac{i-1}{m}}\sigma^2(u)du, 2\sum^m_{i=1}\left(e_{t\pm n-1+\frac{i}{m}}\int^{t\pm n-1+\frac{i}{m}}_{t\pm n-1+\frac{i-1}{m}}\sigma(u)dW(u)\right)+\sum^m_{i=1}e_{s-1+\frac{i}{m}}^2\right]\nonumber\\
&=2\sum^m_{i=1}\sum^m_{j=1}\cov\left[\int^{t-1+\frac{i}{m}}_{t-1+\frac{i-1}{m}}\sigma^2(u)du, e_{t\pm n-1+\frac{j}{m}}\int^{t\pm n-1+\frac{j}{m}}_{t\pm n-1+\frac{j-1}{m}}\sigma(u)dW(u)\right]\\
&\qquad+\sum^m_{i=1}\sum^m_{j=1}\cov\left[\int^{t-1+\frac{i}{m}}_{t-1+\frac{i-1}{m}}\sigma^2(u)du, e^2_{t\pm n-1+\frac{j}{m}}\right]\nonumber\\
&=2f(m)\sum^m_{i=1}\sum^m_{j=1}\cov\left[\int^{t-1+\frac{i}{m}}_{t-1+\frac{i-1}{m}}\sigma^2(u)du, \int^{t-1\pm n+\frac{j}{m}}_{t-1\pm n+\frac{j\pm1}{m}}\sigma(u)du\right].
\end{align}
次に, $\cov[RV_s, u_t]$を目標に, $\cov\left[r_t^2, e^2_{t+\frac{n}{m}}\right], \cov\left[r_t^2, r_{t\pm\frac{n}{m}}e_{t\pm\frac{n}{m}}\right]$を計算していく.
\begin{align*}
%LEM
C^{(4)}_n:=\cov\left[r_t^2,e^2_{t\pm\frac{n}{m}}\right]&=\E\left[r_t^2e^2_{t\pm\frac{n}{m}}\right]-\E\left[r_t^2\right]\E\left[e^2_{t\pm\frac{n}{m}}\right]\\
&=\E\left[r_t^2e^{(1)2}_{t\pm\frac{n}{m}}\right]-\E\left[r_t^2\right]\E\left[e^{(1)2}_{t\pm\frac{n}{m}}\right]\\
\intertext{補題\ref{lem2}より,}
&=
\begin{cases}
2(f(m))^2\E\left[\left(\int^t_{t-\frac{1}{m}}\sigma(s)ds\right)^2\right]&(n=0, 1),\\
0&(n\geq2),
\end{cases}
\end{align*}
\begin{align*}
%LEM
\cov\left[r_t^2, r_{t+\frac{n}{m}}e_{t+\frac{n}{m}}\right]&=\E\left[r_t^2r_{t+\frac{n}{m}}e^{(1)}_{t+\frac{n}{m}}\right]-\E\left[r_t^2\right]\E\left[r_{t+\frac{n}{m}}e^{(1)}_{t+\frac{n}{m}}\right]\\
\intertext{補題\ref{lem2}より,}
&=f(m)\cov\left[\int^{t+\frac{n}{m}}_{t+\frac{n-1}{m}}\sigma^2(u)du, \int^t_{t-\frac{1}{m}}\sigma(u)du\right].
\end{align*}
同様に,
\begin{align*}
\cov\left[r_{t+\frac{n}{m}}^2, r_te_t\right]&=f(m)\cov\left[\int^{t-\frac{n}{m}}_{t-\frac{n-1}{m}}\sigma^2(u)du, \int^t_{t-\frac{1}{m}}\sigma(u)du\right],\\
\cov\left[r_t^2, r_te_t\right]&=f(m)\left(3\E\left[\int^t_{t-\frac{1}{m}}\sigma^2(u)du\int^t_{t-\frac{1}{m}}\sigma(u)du\right]-\cfrac{\sigma^2\E[\sigma(t)]}{m^2}\right).
\end{align*}
これらをまとめて, 
\begin{align*}
C^{(5)}_n:=\cov\left[r_{t+\frac{n}{m}}^2, r_te_t\right]&=
\begin{cases}
f(m)\left(3\E\left[\int^t_{t-\frac{1}{m}}\sigma^2(u)du\int^t_{t-\frac{1}{m}}\sigma(u)du\right]-\cfrac{\sigma^2\E[\sigma(t)]}{m^2}\right)&(n=0),\\
f(m)\cov\left[\int^{t\pm\frac{n}{m}}_{t\pm\frac{n\pm1}{m}}\sigma^2(u)du, \int^t_{t-\frac{1}{m}}\sigma(u)du\right]&(n\geq 1).
\end{cases}
\end{align*}

以上によって,
\begin{align}
\label{rvu}
\cov[RV_t, u_{t+n}]&=\cov\left[\sum^m_{i=1}r^2_{t-1+\frac{i}{m}}, 2\sum^m_{i=1}r_{t+n-1+\frac{i}{m}}e_{t+n-1+\frac{i}{m}}+\sum^m_{i=1}e^2_{t+n-1+\frac{i}{m}}\right]\nonumber\\
&=2\sum^m_{i=1}\sum^m_{j=1}\cov\left[r^2_{t-1+\frac{i}{m}}, r_{t+n-1+\frac{j}{m}}e_{t+n-1+\frac{j}{m}}\right]+\sum^m_{i=1}\sum^m_{j=1}\cov\left[r^2_{t-1+\frac{i}{m}}, e^2_{t+n-1+\frac{j}{m}}\right]\nonumber\\
&=\sum^m_{i=1}\sum^m_{j=1}\left(C^{(4)}_{n+j-i}+2C^{(5)}_{n+j-i}\right)\nonumber\\
&=m\left(C^{(4)}_{mn}+2C^{(5)}_{mn}\right)+\sum^m_{k=1}(m-k)\left(C^{(4)}_{mn+k}+2C^{(5)}_{mn+k}+C^{(4)}_{mn-k}+2C^{(5)}_{mn-k}\right).
\end{align}
Nagakura, Watanabe[2009]から, $\forall s, t$に対して,
\begin{align}
\label{ivd}
\cov[IV_s, d_t]=0.
\end{align}

$d_t=IV_t-RV_t$だから, 式(\ref{ivu}), (\ref{rvu})より,
\begin{align}
\label{du}
\cov[d_t, u_{t+n}]&=\cov[RV_t, u_{t+n}]-\cov[IV_t, u_{t+n}]\nonumber\\
&=\cov[RV_t, u_{t+n}]-2f(m)\sum^m_{i=1}\sum^m_{j=1}\cov\left[\int^{t-1+\frac{i}{m}}_{t-1+\frac{i-1}{m}}\sigma^2(u)du, \int^{t-1\pm n+\frac{j}{m}}_{t-1\pm n+\frac{i\pm1}{m}}\sigma(u)du\right].
\end{align}
\qed
\end{prf}


